Cool Companions to Hot White Dwarfs

We describe a near-IR photometric search for cool red dwarf companions to hot EUV-detected white dwarfs (WDs). While some composite systems have been found optically among WDs detected in recent EUV All-Sky Surveys, we develop an IR technique that probes farther down the main sequence, detecting yet more companions. We use detailed DA model atmosphere fits to optical spectra to predict K magnitudes and distances, against which we contrast our near-IR observations. Our photometric survey reveals 10 DAs with a significant excess in both J and K. Half are newly discovered, and are most likely previously unrecognized binary systems. Neither the frequency of infrared excess nor the mass estimate of the red dwarf companion correlate with white dwarf mass, as might be expected if either the EUV detectability or mass of the white dwarfs were significantly affected by a companion. Infrared spectra of these systems should help to determine the mass and spectral type of the cool companions presumably causing the IR excess, leading to better estimates of the mass ratio distribution in binaries. Counting previously known binaries, and resolved pairs, we find the total binary fraction of the sample is at least a third. Since most WD progenitors had initial masses larger than about 2 solar masses, we thus provide a photometric measure of the binary fraction of high mass stars that would be difficult to perform in high mass main sequence stars. We estimate that 90% of the companions are of type K or later.

==> tabpjg1.tex <==
%\documentstyle[12pt,aasms4]{article}
%\begin{document}

\begin{deluxetable}{lllrllll}
\tablewidth{0cm}
\tablecaption{SAMPLE OF EUV-SELECTED DA WHITE DWARFS
\label{tsample}}
\tablehead{
 \colhead{REJ}
&\colhead{Other Names}
&\colhead{$V$}
&\colhead{$\teff$}
&\colhead{$\log g$}
&\colhead{$M/M_\odot$}
&\colhead{Refs}
&\colhead{Notes} \\
%
\colhead{ } 
&\colhead{ }  
&\colhead{ }  
&\colhead{ }  
&\colhead{ }  
&\colhead{ }  
&\colhead{ } 
&\colhead{ }  
}
%  REJ     OtherNames                  V       Teff    logg  M  Refs Notes
\startdata
0007+331$^a$   & GD\,2              & 13.85 & 45653 & 7.77 & 0.57 & 1,2 & \\ 
0134$-$160$^a$ & GD\,984, PHL\,1043 & 13.96 & 43722 & 7.70 & 0.54 & 1,2,9  & DA+dM \\
0138+252       & PG\,0136+251       & 15.87 & 38964 & 9.00 & 1.22   & 1,1 & peculiar\\   
0148$-$253$^a$ & GD\,1401           & 14.69 & 25707 & 7.70 & 0.50 & 1,2,6  & NS, DA+dM \\
0235+034       & Feige\,24          & 12.56 & 62947 & 7.53 & 0.54 & 1,1,13 & DAe+dM \\   
%V=12.42, J=11.22, H=10.67, K= 10.44 in Probst 1983
0237$-$122$^a$ & PHL\,1400          & 14.92 & 31570 & 8.38 & 0.85 & 1,2  & \\
0348$-$005     & GD\,50             & 14.04 & 38881 & 8.97 & 1.17    & 1,2  & \\
0350+171       & V471\,Tau          & 13.65 & 34200 & 8.80 & 1.12 & 1,1 & DA+K0  \\
%0415$-$073     & 40\,Eri\tablenotemark{b}  &  9.50  & 15490 & 7.77 & 0.50 & 7,6 & K14+DA+M4.5 \\
%V=9.31, J=6.68, H=6.15, K=5.90  in Probst 1983
0427+740$^{a}$   &               & 15.9   & 47549 & 7.84 & 0.61 & 3,2  & visual pair, 8\arcsec \\  
0443$-$034$^a$ &               & 16.9   & 65140 & 9.12 & 1.29  & 3,4  & \\
0457$-$280$^a$ & MCT\,0455$-$2812 & 13.95  & 50061 & 7.63 & 0.53  & 1,2  & NS \\
0512$-$004$^a$ &               & 14.2   & 31333 & 7.34 & 0.45 & 3,2  & \\
0521$-$102$^a$ &               & 15.81  & 32775 & 8.53 & 0.94 & 1,2  & \\
% WHY NOT USE NGS FITS HERE FOR 0521? WHAT YOU LIST IS VENNES' FIT.
%0550-240      &               & 16.371 & 51870 & 7.29 & 0.44  & 1,1 & NS  \\
0827+288       & PG\,0824+289  & 14.22  & 51934 & 8.00 & 0.70  & 1,1,12 & DA+dC+M3V \\
0841+032$^a$   &               & 14.47  & 37687 & 7.68 & 0.52 & 1,2  & \\
0845+488       & HD74389B      & 15.5:  & 39500 & 8.04 & 0.65  & 7,5 & DA+A2V \\
0902$-$040$^a$ &               & 13.19  & 22285 & 7.76 & 0.51 & 1,2  & \\
0907+505$^a$   & PG\,0904+511  & 16.54  & 31791 & 8.04 & 0.66 & 1,2  & \\
%\tablebreak
0916$-$194$^a$ &               & 17.3   & 56400 & 9.12 & 1.29  & 3,4 & visual pair, 6.4\arcsec \\  
0940+502$^a$   & PG\,0937+506  & 16.0   & 35511 & 7.62 & 0.51 & 3,2 & \\
0957+852$^a$   &               & 15.4   & 50205 & 8.29 & 0.82 & 3,2 & \\
1016$-$052     &               & 14.21  & 53827 & 8.08 & 0.65  & 1,1,4 & DA+dM \\
1019$-$140$^a$ &               & 14.93  & 31100 & 7.85 & 0.57 & 1,2 & \\
1029+450$^a$   & PG\,1026+454  & 16.13  & 35017 & 7.64 & 0.51 & 1,2 & \\
1032+532$^a$   &               & 14.45 & 42785 & 7.89 & 0.62 & 1,2 & \\
1033$-$114     & G\,162$-$66, LTT\,3870 & 13.01  & 23741 & 7.79 & 0.52 & 1,2  & \\
%V=12.97, K= 13.79\pm0.08 in Probst 1983
1036+460$^a$   & GD\,123 & 14.34  & 28720 & 7.95 & 0.61 & 1,2,10  & DA+K \\
%K= 11.79 in Zuckerman and Becklin 1992
1043+490$^a$   &               & 16.23  & 40461 & 7.87 & 0.60    & 1,2,14  & visual pair, 8\arcsec \\
1043+445$^a$   & PG\,1040+451  & 16.94  & 48000 & 7.98  & 0.63 & 3,4  & \\  
1044+574$^a$   & PG\,1041+580  & 14.64  & 29878 & 7.73 & 0.52 & 1,2  & \\
1100+713$^a$   & PG\,1057+719  & 14.68  & 40328 & 7.75 & 0.55 & 1,2  & \\
1112+240$^a$   & Ton\,61       & 15.77  & 39281 & 7.71 & 0.53 & 1,2  & \\
1122+434$^a$   & PG\,1120+439  &  15.8  & 26152 & 8.23 & 0.75 & 3,2  & \\
1126+183$^a$   & PG\,1123+189  & 14.13 & 52747 & 7.69 & 0.56 & 1,2,10  & DA+dM\\
%K= 11.95 in Zuckerman and Becklin 1992
1128$-$025$^a$ & PG\,1125$-$026& 15.73  & 30227 & 8.15 & 0.71 & 1,2  & \\
1148+183$^a$   & PG\,1145+188  & 14.33  & 24717 & 7.84 & 0.55 & 1,2  & \\
1235+233$^a$   & PG\,1232+238  & 17.4   & 45639 & 7.77 & 0.57   & 3,2  & \\
1236+475$^a$   & PG\,1234+482  & 14.38  & 55570 & 7.57 &  0.53  & 1,1  & reclassified DB \\
1257+220$^a$   & GD\,153       & 13.38  & 38324 & 7.71 & 0.53 & 2  & \\
1316+295       & HZ\,43        & 12.99  & 49000 & 7.70 & 0.56 & 1,8 & DA+dM \\
%V=12.86, J=10.35, H=9.8, K=9.52  in Probst 1983
1336+694$^a$   & PG\,1335+701  & 15.4   & 29067 & 8.27 & 0.78 & 3,2  & \\
1426+500       &               & 13.6   & 29800 & 7.98 & 0.60 & 3,4,6 & DA+MVe \\
1431+370$^a$   & GD\,336       & 15.27  & 33988 & 7.86 & 0.58 & 1,2  & \\
1440+750$^a$   &               & 15.32  & 42400 & 8.54 & 0.96  & 3,4  & \\
1446+632$^a$   &               & 16.4   & 37340 & 7.72 & 0.53 & 3,2  & \\
\tablebreak   
1629+780$^a$   &               & 13.03  & 39882 & 7.88 & 0.61 & 1,2,11 & DA+M4V \\
% See also Sion et al. 1995
1638+350$^a$   & PG\,1636+351  & 14.83  & 34879 & 7.90 & 0.61 & 1,2  & \\
1643+411$^a$   & PG\,1642+414  & 16.2   & 28240 & 8.15 & 0.71 & 3,2 & \\
1650+403$^a$   &               & 15.83  & 37698 & 7.90 & 0.61 & 1,2  & \\
1659+440$^a$   & PG\,1658+440  & 14.62  & 30510 & 9.36 & 1.31 & 3,5  & magnetic DA \\ 
1711+664$^a$   &               & 17.10  & 47994 & 8.78 & 1.09 & 1,2 & visual pair, 2.5\arcsec\\
1726+583$^a$   & PG\,1725+586  & 15.45   & 52413 & 8.14 & 0.75 & 1,2  & visual pair, 6.7\arcsec\\
1800+683$^a$   & KUV\,18004+6836 & 14.74 & 43868 & 7.74 & 0.56   & 1,2  & \\
1820+580$^a$   &               & 13.95  & 43296 & 7.70 & 0.54 & 1,2 & \\
1845+682$^a$   & KUV\,18453+6819 & 15.5 & 35599 & 8.15 & 0.72   & 3,2 & \\
2116+735$^a$   & KUV\,21168+7338 & 15.0 & 49777 & 7.65 & 0.54  & 3,2  & \\
2126+192       & IK\,Peg       &  6.07  & \ldots  & \ldots  & \ldots  & \ldots  & DA+A8m \\
%2127$-$221    &               & 14.66  & 48297 & 7.69 & 0.55  & 1,1 & NS    \\
2207+252       &               & 14.58  & 26129 & 8.20 & 0.74 & 1,2 &  visual pair, 8.9\arcsec\\
%2210$-$300    &               & 14.79  & 28268 & 7.60 & 0.46 & 1,1 &  NS \\
2312+104$^a$   & GD\,246       & 13.09  & 51950 & 7.76 & 0.59 & 1,2 & \\
%NS 23 53 07.0 -24 32 12  MCT2350-2448  15.10  DA1       
\enddata
\tablenotetext{a}{New IR photometry presented in this work.}
%\tablenotetext{b}{DA WD 40~Eri~B is probably not the EUV
%source. 40~Eri~c is.}
\tablenotetext{}{NOTES: NS means not in official sample, but may have
optical fits in NGS99 and/or IR data.  Visual pairs within 10\arcsec
and $\Delta R=3$mag are noted with separations.} 
\tablenotetext{}{REFERENCES: First reference is for $V$ mag,
2d for $\teff$, $\log g$, and $M/M_\odot$; 3d if listed is for
companion's spectral type and/or mass of previously known companion.
If a multiple system has no third reference listed, it has
several references available in SIMBAD.
(1) - Marsh et al. 1997;
(2) - NGS99;
(3) - V from McCook and Sion;
(4) - Vennes et al. 1997; % ApJ, 480, 714
(5) - Schmidt et al. 1992;
(6) - FKB 1997;
(7) - SIMBAD;
(8) - Napiwotski, R. et al. 1993; 
(9) - Bues \& Aslan 1995;  
(10) - Green, Schmidt \& Liebert 1986;
(11) - Catal\`an et al. 1995;
(12) - Green \& Margon 1994;
(13) - Vennes \& Thorstensen 1994; % AJ, 108,1881
(14) - Schwartz et al. 1995.
}
\end{deluxetable}

%\end{document}

 


==> tabpjg2.tex <==
%\documentstyle[apjpt4]{article}

% This example of a table uses the AASTeX "deluxetable" environment.  Used
% with either the apjpt4 or aj_pt4 style file, this table environment produces
% camera-ready tables that are ready to be photographed for publication.
%

%\begin{document}

\begin{deluxetable}{ccp{4cm}cp{4cm}}
%\tablenum{}
\tablewidth{0pt}
\tablecaption{Summary of Observing Runs\label{tbl-obsrun}}
\tablehead{
\colhead{ID} & 
\colhead{UT date}  & 
\colhead{Standard Stars} &
\colhead{Standard Stars} &
\colhead{Conditions} \\
\colhead{} &
\colhead{} &
\colhead{used\tablenotemark{a}} &
\colhead{References\tablenotemark{b}} &
\colhead{}
}
\startdata
KP01 & 
04 Jan 96 & 
FS \#6, \#10, \#19, LHS 254, LHS 325 & 
1,2 & 
Clear or light cirrus.\\
KP02 & 
05 Jan 96 &
FS \#10, \#19, LHS 191, LHS 2347 &
1,2 &
Cirrus, but eventually very clear. \\
KP03 & 
06 Jan 96 &
FS \#2, \#10, \#19, LHS 2502 &
1,2 &
Heavy cirrus. \\
KP04 & 
07 Jan 96 &
FS \#15, \#10, \#19, LHS 191 &
1,2 &
High thin cirrus. \\
KP05 &
02 July 96 &
\nodata &
\nodata &
Cloudy, no data. \\
KP06 &
03 July 96 &
\nodata &
\nodata &
Cloudy, no data. \\
KP07 &
04 July 96 &
\nodata &
\nodata &
Cloudy, no data. \\
KP08 &
05 July 96 &
\nodata &
\nodata &
Cloudy, no data. \\
KP09 &
06 July 96 &
\nodata &
\nodata &
Cloudy, no data. \\
KP10 &
29 Oct 96 &
FS \#1,\#6, \#9, \#12, \#15, \#29, \#31 &
1 &
Mostly clear. \\
KP11 &
30 Oct 96 &
FS \#1, \#10, \#14, \#29, GJ 1057, GJ 1002 &
1,2 &
Photometric. \\
KP12 &
20 Jan 98 &
\nodata &
\nodata &
Cloudy. \\
KP13 &
21 Jan 98 &
\nodata &
\nodata &
Fog.  Telescope closed. \\
KP14 &
22 Jan 98 &
FS \#2, \#6, \#21, \#24, \#18, \#19 &
1 &
Clear. \\
KP15 &
09 May 98 &
FS \#21, \#23, \#24, \#27, \#29, \#33 &
1 &
Clear. \\
KP16 &
10 May 98 &
FS \#16, \#20, \#21, \#23, \#35 &
1 &
Mostly clear with moderate haze. \\
KP17 &
11 May 98 &
FS \#19, \#21, \#27 &
1 &
Hazy
\tablenotetext{a}{FS=UKIRT faint star}
\tablenotetext{b}{STANDARD STAR REFERENCES:
(1) - Casali \& Hawarden 1992; (2) - Leggett 1992}
\enddata
\end{deluxetable}

%\end{document}


==> tabpjg3.tex <==
%\documentstyle[apjpt4]{article}

% This example of a table uses the AASTeX "deluxetable" environment.  Used
% with either the apjpt4 or aj_pt4 style file, this table environment produces
% camera-ready tables that are ready to be photographed for publication.
%

%\begin{document}

\begin{deluxetable}{cll}
%\tablenum{}
\tablewidth{5in}
\tablecaption{Summary of Target Observations\label{tbl-obs}}
\tablehead{
\colhead{Target} &
\colhead{Observing Runs} &
\colhead{Notes$^a$}
}
\startdata
0007+331 & KP02, KP04, KP10 & \\
0134$-$160 & KP02, KP04, & \\
         & KP10  & jn3 \\
0148$-$253 & KP02, KP03, KP04 & \\
0237$-$122 & KP04, & \\ 
         & KP10  & kn9 \\
0348$-$005 & KP01, KP02, KP03, KP04, & \\ 
         & KP11  & jn3, kn3 \\
0427+740 & KP01, KP03, KP04, & \\
         & KP14  & kn9 \\
0443$-$034 & KP03, & \\
         & KP11  & jn9, kn9 \\
0457$-$280 & KP03, KP11 & \\
0512$-$004 & KP01, KP03, KP04, KP10, & \\ 
         & KP14  & jn9, kn9 \\
0521$-$102 & KP01, KP03, & \\ 
         & KP10, & jn9, kn9 \\
         & KP14  & kn9 \\
0827+284 & KP11  & \\
0841+032 & KP01, KP10, & jn9, kn9 \\
         & KP14  & kn9 \\
0902$-$040 & KP01, KP04 & \\
         & KP10  & kn9 \\
0907+505 & KP03, KP04, KP11, KP14, & jn9, kn9 \\
         & KP17  & kn18 \\
0916$-$194 & KP02  & jn9, kn9 \\
0940+502 & KP01, & jn9, kn9 \\ 
         & KP15, & jc1, kc1 \\
         & KP16, & jc2, jn9, kc2, kn9 \\
         & KP17  & kc9, kn18 \\
0957+852 & KP02, & \\
         & KP14, & kn9 \\
         & KP16, & jc2, jn9, kc2, kn9 \\
         & KP17  & kc9, kn9 \\
1019$-$140 & KP02  & \\
1029+450 & KP02  & \\
1032+532 & KP01, KP04, & \\
         & KP14  & kn9 \\
1033$-$114 & KP01, KP02, KP03, KP04 & \\
1036+460 & KP02  & \\
1040+451 & KP15, & jc1, jn12, kc1, kn12 \\
         & KP16, & jc2, jn9, kc2, kn9 \\
         & KP17  & kc12 \\
\tablebreak
1043+490 & KP02, & \\
         & KP14, & kn9 \\
         & KP15, & jc1, jn9, kc2, kn9 \\
1044+574 & KP02  & \\
1100+713 & KP02, & \\
         & KP17  & kn15 \\
%1112+240 & KP14  & kn9 \\
1112+240 & KP16  & jc2, jn9, kc2, kn9 \\
1122+434 & KP02, & \\
         & KP16  & jc2, kc2, kn9 \\
1126+183 & KP01, KP04 \\
1128$-$025 & KP02, & \\
         & KP16  & jc1, kc1 \\
1148+183 & KP01, KP03 & \\
1235+233 & KP14, & kn9 \\
         & KP16, & jc2, jn9, kc3, kn9 \\
         & KP17, & kc12, kn9 \\
1234+482 & KP14  & kn9 \\
1257+220 & KP01, KP02, KP03 & \\
1336+694 & KP03, KP04, & \\ 
         & KP14, & kn9 \\
         & KP16  & jc1, jn9, kc2, kn9 \\
1431+370 & KP03, KP04 & \\
1431+370 & KP10, & kn9 \\ 
         & KP16, & kn9,jn9,jc1,kc2 \\
         & KP17  & kn9,kc12 \\
1440+750 & KP14, & \\
         & KP16, & jc1, jn9, kc2, kn9 \\
         & KP17  & kc12, kn9 \\
1446+632 & KP14, & \\
         & KP16, & jc2, jn9, kc3, kn15 \\
         & KP17  & kc12, kn9 \\
1629+780 & KP15  & jc1, kc1 \\
1638+350 & KP15  & jc1, kc1, kn9 \\
1643+411 & KP15, & jc1, jn9, kc2, kn9 \\
         & KP16, & jc2, jn9, kc3, kn15 \\
         & KP17  & kc12, kn9 \\
1650+403 & KP15, & jc1, jn9, kc1, kn9 \\
         & KP16  & jc2, jn9, kc2, kn9 \\
1658+441 & KP14, & \\
         & KP15, & jc1, jn9, kc1, kn9 \\
         & KP16, & jc2, kn9, kc2, kn9 \\
         & KP17  & kc12, kn9 \\
1711+664 & KP15  & jc1, jn18, kc1, kn9 \\
1726+583 & KP15  & jc1, jn9, kc1, kn9 \\
\tablebreak
1800+683 & KP15, & jc1, jn9, kc1, kn9 \\
         & KP16, & jc2, jn9, kc2, kn9 \\
         & KP17, & kc12, kn9 \\
1820+580 & KP11, & \\
         & KP15  & jc1, jn9, kc1, kn9 \\
1845+682 & KP11, & \\
         & KP15  & jc1, jn9, kc1, kn9 \\
2116+735 & KP10, KP11, & \\
         & KP15, & jc1, jn9, kc1, kn9 \\
         & KP16, & jc2, jn9, kc3, kn9 \\
         & KP17  & kc12, kn9 \\
2127$-$221 & KP10  & jn9, kn9 \\
2207+252 & KP15, & jc1, jn9, kc1, kn9 \\
         & KP17  & \\
2312+104 & KP02, KP03, KP04 & \\
2353$-$243 & KP10  & jn9, kn9 \\
%ton61    & KP16  & jc2, jn9, kc2, kn9 \\
%warren 1 & KP11  & jn9 \\
%warren 2 & KP11  & jn9 \\
\enddata
\tablenotetext{a}{The number of 10sec co$-$adds per
exposure in both $J$ and $K$ bands is nominally 6, and the number of
dithered exposures is also 6, except as noted in the Notes.}
\tablenotetext{}{} 
\tablenotetext{}{NOTES:} 
\vskip0.1cm
\tablenotetext{}{$X$c$Y$ denotes that in the $X$ bandpass 
the number of co-adds performed per exposure is $Y$
(e.g., jc1 means 1 co-add per exposure in {\it J}\
band).}
\tablenotetext{}{$X$n$Y$ denotes that in the $X$ bandpass
the number of combined dithered exposures is $Y$
(e.g., kn9 means 9 dithered exposures combined in the {\it K}\ band).}
\end{deluxetable}

%\end{document}


==> tabpjg4.tex <==
%\documentstyle[apjpt4]{article}
%\begin{document}

\begin{deluxetable}{lccccrc|rcccl}
\tablewidth{0cm}
\tablecaption{Observed and Predicted Magnitudes and Colors of DA White Dwarf Stars
\label{tirdata}}
\tablehead{
 \colhead{RE Name}
&\colhead{$J$}
&\colhead{$\sigma_J$}
&\colhead{$K$}
&\colhead{$\sigma_K$}
&\colhead{$(J-K)$}
&\colhead{$\sigma_{(J-K)}$}
&\colhead{$M_V$}
&\colhead{$(V-K)_p$}
&\colhead{$J_p$}
&\colhead{$K_p$}
&\colhead{Notes} \\
%
\colhead{ } 
&\multicolumn{6}{c}{observed}
&\multicolumn{4}{c}{predicted}
&\colhead{ }  
}
%    name       J        err       K        err      J-K      err     Mv        J       K       J-K   Notes
\startdata
 0007$+$331 &  14.62 &   0.02 &  14.82 &  0.07 & $-$0.21 &   0.07 &   9.06 & $-$0.72 &  14.33 &  14.57 &   \\ 
{\bf 0134$-$160} &  12.95 &   0.01 &  12.21 &  0.01 &    0.74 &   0.01 &   9.00 & $-$0.72 &  14.43 &  14.68 &   \\ 
{\bf 0148$-$253} &  12.33 &   0.01 &  11.56 &  0.04 &    0.76 &   0.04 &   9.98 & $-$0.60 &  15.08 &  15.29 &   \\ 
 0237$-$122 &  15.74 &   0.06 &  15.93 &  0.12 & $-$0.18 &   0.14 &  10.68 & $-$0.68 &  15.36 &  15.60 &   \\ 
 0348$-$005 &  14.80 &   0.06 &  14.66 &  0.52 &    0.14 &   0.52 &  11.46 & $-$0.71 &  14.50 &  14.75 & 1 \\ 
{\bf 0427$+$740} &  15.64 &   0.03 &  15.62 &  0.12 &    0.02 &   0.12 &   9.13 & $-$0.73 &  16.38 &  16.63 &   \\ 
 0443$-$034 &  17.38 &   0.05 &  17.99 &  0.07 & $-$0.61 &   0.08 &  11.23 & $-$0.75 &  16.49 &  16.75 &   \\ 
 0457$-$280 &  14.62 &   0.02 &  14.80 &  0.03 & $-$0.18 &   0.03 &   8.69 & $-$0.73 &  14.43 &  14.68 &   \\ 
 0512$-$004 &  14.43 &   0.03 &  14.67 &  0.01 &    0.15 &   0.40 &   8.81 & $-$0.67 &  14.63 &  14.87 &   \\ 
 0521$-$102 &  16.76 &   0.20 &  17.13 &  0.13 & $-$0.37 &   0.24 &  10.87 & $-$0.69 &  16.26 &  16.50 &   \\ 
 0550$-$240 &  16.93 &   0.10 &  17.28 &  0.41 & $-$0.34 &   0.42 &   9.03 & $-$0.73 &  17.18 &  17.43 &   \\ 
 0841$+$032 &  15.17 &   0.02 &  15.49 &  0.01 & $-$0.33 &   0.02 &   9.17 & $-$0.70 &  14.93 &  15.18 &   \\ 
 0902$-$040 &  13.70 &   0.01 &  13.90 &  0.05 & $-$0.20 &   0.05 &  10.37 & $-$0.53 &  13.54 &  13.72 &   \\ 
 0907$+$505 &  17.16 &   0.10 &  17.54 &  0.64 & $-$0.39 &   0.65 &  10.09 & $-$0.68 &  16.98 &  17.22 &   \\ 
{\bf 0916$-$194} &  13.94 &   0.02 &  13.64 &  0.04 &    0.36 &   0.10 &  11.36 & $-$0.74 &  17.78 &  18.04 &   \\ 
 0940$+$502 &  16.73 &   0.07 &  16.97 &  0.02 & $-$0.24 &   0.07 &   9.14 & $-$0.70 &  16.45 &  16.70 &   \\ 
 0957$+$852 &  16.49 &   0.08 &  16.72 &  0.09 & $-$0.23 &   0.12 &   9.87 & $-$0.73 &  15.88 &  16.13 &   \\ 
 1019$-$140 &  15.17 &   0.04 &  15.45 &  0.14 & $-$0.28 &   0.14 &   9.82 & $-$0.67 &  15.36 &  15.60 &   \\ 
 1029$+$450 &  16.92 &   0.09 &  17.54 &  0.70 & $-$0.62 &   0.71 &   9.20 & $-$0.69 &  16.58 &  16.82 &   \\ 
 1032$+$532 &  15.38 &   0.01 &  15.45 &  0.11 & $-$0.07 &   0.11 &   9.35 & $-$0.72 &  14.92 &  15.17 &   \\ 
 1033$-$114 &  14.80 &   0.06 &  14.66 &  0.52 &    0.14 &   0.52 &  10.31 & $-$0.56 &  13.38 &  13.57 &   \\ 
%K= 13.79\pm0.08 in Probst 1983
{\bf 1036$+$460} &  12.62 &   0.04 &  11.89 &  0.09 &    0.72 &   0.10 &   9.95 & $-$0.65 &  14.76 &  14.99 &   \\ 
%K= 11.79 in Zuckerman and Becklin 1992
 1043$+$490 &  16.86 &   0.02 &  16.95 &  0.22 & $-$0.10 &   0.22 &   8.40 & $-$0.72 &  16.71 &  16.95 &   \\ 
 1043$+$445 &  18.00 &   0.05 &  17.48 &  0.09 &    0.52 &   0.11 &   9.43 & $-$0.73 &  17.42 &  17.67 &   \\ 
 1044$+$574 &  15.32 &   0.04 &  15.73 &  0.17 & $-$0.42 &   0.18 &   9.72 & $-$0.66 &  15.06 &  15.30 &   \\ 
 1100$+$713 &  15.51 &   0.10 &  15.78 &  0.17 & $-$0.27 &   0.20 &   9.19 & $-$0.71 &  15.14 &  15.39 &   \\ 
 1112$+$240 &  16.37 &   0.21 &  16.51 &  0.55 & $-$0.14 &   0.59 &   9.17 & $-$0.71 &  16.24 &  16.48 &   \\ 
 1122$+$434 &  16.12 &   0.05 &  16.39 &  0.34 & $-$0.27 &   0.34 &  10.82 & $-$0.61 &  16.20 &  16.41 &   \\ 
{\bf 1126$+$183} &  12.74 &   0.09 &  12.04 &  0.10 &    0.70 &   0.14 &   8.47 & $-$0.73 &  14.61 &  14.86 &   \\ 
 1128$-$025 &  16.18 &   0.06 &  16.48 &  0.17 & $-$0.30 &   0.18 &  10.38 & $-$0.67 &  16.16 &  16.40 &   \\ 
 1148$+$183 &  14.96 &   0.06 &  15.22 &  0.20 & $-$0.26 &   0.20 &  10.31 & $-$0.58 &  14.71 &  14.91 &   \\ 
\tablebreak	
 1235$+$233 &  18.31 &   0.11 & \ldots & \ldots & $-$2.36 &   0.28 &   9.06 & $-$0.72 &  17.88 &  18.12 & 2 \\ 
 1236$+$475 &  14.91 &   0.06 &  14.90 &  0.16 &    0.01 &   0.17 &   8.37 & $-$0.73 &  14.86 &  15.11 &   \\ 
 1257$+$220 &  14.17 &   0.06 &  14.43 &  0.02 & $-$0.26 &   0.05 &   9.21 & $-$0.71 &  13.84 &  14.09 &   \\ 
 1336$+$694 &  15.85 &   0.02 &  16.12 &  0.04 & $-$0.28 &   0.04 &  10.66 & $-$0.65 &  15.82 &  16.05 &   \\ 
 1431$+$370 &  15.97 &   0.04 &  16.37 &  0.16 & $-$0.40 &   0.17 &   9.65 & $-$0.69 &  15.72 &  15.97 &   \\ 
 1440$+$750 &  17.21 &   0.11 &  16.64 &  0.12 &   0.57 &   0.16 &  11.39 &  $-$0.70 &  15.77 &  16.02 &   \\ 
 1446$+$632 &  16.77 &   0.11 &  17.77 &  0.07 &  $-$1.00 &   0.12 &   9.26 &  -0.70 &  16.86 &  17.10 &   \\ 
{\bf 1629$+$780} &  10.96 &   0.03 &  11.19 &  0.04 & $-$0.23 &   0.05 &   9.42 & $-$0.71 &  13.49 &  13.74 &   \\ 
 1638$+$350 &  15.55 &   0.11 &  15.57 &  0.64 & $-$0.01 &   0.64 &   9.67 & $-$0.70 &  15.28 &  15.53 &   \\ 
 1643$+$411 &  16.86 &   0.10 &  17.46 &  0.05 & $-$0.61 &   0.11 &  10.53 & $-$0.64 &  16.62 &  16.84 &   \\ 
 1650$+$403 &  16.60 &   0.08 &  16.86 &  1.05 & $-$0.26 &   1.05 &   9.54 & $-$0.71 &  16.29 &  16.54 &   \\ 
 1658$+$441 &  15.47 &   0.10 &  15.68 &  0.02 & $-$0.21 &   0.10 &  12.70 & $-$0.67 &  15.06 &  15.29 &   \\ 
{\bf 1711$+$664} &  15.02 &   0.01 &  14.19 &  0.18 &    0.83 &   0.18 &  10.84 & $-$0.73 &  17.58 &  17.83 &   \\ 
 1726$+$583 &  16.40 &   0.26 &  16.17 &  1.51 &    0.23 &   1.53 &   9.56 & $-$0.73 &  15.93 &  16.18 &   \\ 
 1800$+$683 &  15.54 &   0.04 &  15.87 &  0.04 & $-$0.33 &   0.06 &   9.06 & $-$0.72 &  15.21 &  15.46 &   \\ 
{\bf 1820$+$580} &  14.07 &   0.04 &  13.42 &  0.01 &    0.65 &   0.04 &   9.01 & $-$0.72 &  14.42 &  14.67 &   \\ 
{\bf 1845$+$682} &  14.85 &   0.10 &  14.37 &  0.19 &    0.47 &   0.22 &  10.06 & $-$0.70 &  15.95 &  16.20 &   \\ 
 2116$+$735 &  15.54 &   0.01 &  15.93 &  0.06 & $-$0.39 &   0.06 &   8.74 & $-$0.73 &  15.48 &  15.73 &   \\ 
 2207$+$252 &  14.34 &   0.08 &  14.06 &  0.22 &    0.28 &   0.23 &  10.77 & $-$0.61 &  14.98 &  15.19 & 3 \\ 
 2312$+$104 &  13.81 &   0.04 &  14.06 &  0.01 & $-$0.14 &   0.75 &   8.88 & $-$0.73 &  13.57 &  13.82 &   \\ 
\enddata
\tablenotetext{}{NOTES: Objects with significant IR excess, are
shown in boldface.}
\tablenotetext{1}{Faint IR standard star - photometry from Casali \&
 Hawarden (1992)}
\tablenotetext{2}{Object is barely discernible on $K$ band image;
$K$ photometry unreliable.}
\tablenotetext{3}{IR photometry known to include nearby optically
resolved object at 2.2\arcsec}
\end{deluxetable}



==> tabpjg5.tex <==
%\documentstyle[apjpt4]{article}
%\begin{document}

\begin{deluxetable}{lcccllcl}
\tablewidth{0cm}
       \tablecaption{Derived Properties of Candidate Cool Companions
\label{tcompanions}}
\tablehead{
\colhead{REJ Name}
&\colhead{$J_c$}
&\colhead{$K_c$}
&\colhead{$M_{K_c}$}
&\multicolumn{2}{c}{M Subtype$^a$} 
&\colhead{$V_c^b$}
&\colhead{Notes} \\
%
\colhead{ }  
&\colhead{ }  
&\colhead{ }  
&\colhead{ }  
&\colhead{(YD) }  
&\colhead{(OD) }  
&\colhead{(OD) }  
&\colhead{ }  
}
% name         Jc       Kc     Mkc    M Subtype       Vc    Notes
%                                    YD    OD   

\startdata
0134$-$160 &  13.3 &  12.3 &  7.4 & 4.5 & 3.5  &  17.4  & 1 \\ 
0148$-$253 &  12.4 &  11.6 &  6.9 & 4   & 3    &  16.4  & 1 \\ 
0427$+$740 &  16.4 &  16.2 &  9.4 & 6.5 & 6    &  23.5  & 3 \\ 
0916$-$194 &  14.0 &  13.7 &  7.7 & 5   & 4    &  19.2  &   \\ 
1036$+$460 &  12.8 &  12.0 &  7.6 & 5   & 4    &  17.3  & 1 \\ 
1126$+$183 &  13.0 &  12.1 &  6.5 & 3.5 & 2.5  &  16.6  & 1 \\ 
1629$+$780 &  11.1 &  11.3 &  7.7 & 5   & 4    &  16.6  & 1 \\ 
1711$+$664 &  15.1 &  14.2 &  8.0 & 5.5 & 5    &  20.0  & 2 \\ 
1820$+$580 &  15.5 &  13.8 &  8.9 & 6   & 5.5  &  21.0  &   \\ 
1845$+$682 &  15.3 &  14.6 &  9.2 & 6.5 & 6    &  21.9  &   \\ 
%2207$+$252 &  15.2 &  14.5 & 10.7 & 9   & 9    &  23.4  & 2 \\ 
\enddata
\tablenotetext{a}{Approximate spectral type from $M_{K_c}$ and Leggett
(1992) Table~6, for Young Disk and Old Disk stars. }
\tablenotetext{b}{Approximate $V$ magnitude of companion assuming Old
Disk population, from $M_{K_c}$ and $(V-K)$ of Leggett
(1992) Table~6.} 
\tablenotetext{}{NOTES:  
1) Known binary; see Table~\ref{tsample}. \\
2) IR photometry known to include nearby marginally optically-resolved
object at separation indicated in Table~\ref{tsample}. \\ 
3) This star is spatially resolved at near-IR wavelengths, with a
companion within $<2\arcsec$.  Some nebulosity (diffuse emission) is
also noted nearby. The more distant companion noted in Table~\ref{tsample}
is not included in the IR photometry.} 
\end{deluxetable}






